Leveraging Semantic Web Search and Browse Sessions for Multi-Turn Spoken Dialog Systems

Training statistical dialog models in spoken dialog systems (SDS) requires large amounts of annotated data. The lack of scalable methods for data mining and annotation poses a significant hurdle for state-of-the-art statistical dialog managers. This paper presents an approach that directly leverage billions of web search and browse sessions to overcome this hurdle. The key insight is that task completion through web search and browse sessions is (a) predictable and (b) generalizes to spoken dialog task completion. The new method automatically mines behavioral search and browse patterns from web logs and translates them into spoken dialog models. We experiment with naturally occurring spoken dialogs and large scale web logs. Our session-based models outperform the state-of-the-art method for entity extraction task in SDS. We also achieve better performance for both entity and relation extraction on web search queries when compared with nontrivial baselines.

==> expSetup.tex <==
We apply our query session based model on two main tasks -- \textit{web query semantic parsing} and \textit{statistical dialog management}.


\subsection{Data}

\subsubsection{The Knowledge Base -- Satori}
\todo{decsription of Satori}

\subsubsection{Web Search Query-Click Log (IE log)}
We collect 12 weeks' web search query-click logs based on IE browsing history, which spans from March 18, 2013 to June 09, 2013. This dataset will be called ``IE log" henchforth. Among the 12 weeks' IE log, 80\% of the data is randomly selected as the training data for both tasks.

\todo{show the statistics on the dataset}

\subsubsection{Conversational Browsing Data (CB data)}
\todo {description of the dataset}
\todo{show the statistics on the dataset}

\subsubsection{Conversational Browsing on Netflix (Netflix data)}
\todo {description of the dataset}
\todo{show the statistics on the dataset}

\subsection{Task 1: Web Query Semantic Parsing}
\quesiton {we might want to give some description about this task in the introduction.}

Based on the investigation from \cite{Pound:2012:IKQ:2396761.2396803}, three most frequently occurring templates (or types) of queries dominate the entity-based web search (i.e. more than 65\% of the sampled queries fall in these three types). The three templates are:

\begin{itemize}
\item
Entity
\item
Type $\sqcap$ Relation(Entity)
\item
Entity$_{0}$ $\sqcap$ Relation(Entity$_{1}$)
\end{itemize}

In this study, we focus on improving the semantic parsing performance for queries that match these three most frequent templates by leveraging history information in the query session.

We compare with one baseline based on gazetteer matching and one supervised method based on Maximum Entropy \cite{Berger:1996:MEA:234285.234289} with the same set of features used in our session-based model.


\subsection{Task 2: Statistical Dialog Management}
\quesiton {same here -- we might want to give some description about this task in the introduction, like what is the belief update, and how it is represented as \{entity, relation, type, etc\}}


This set of experiments are conducted on both CB data and Netflix data.

We compare with the same baseline in web query semantic parsing and the state-of-the-art approach designed for the same task in dialog management from \cite{HeckEtAl2013}.






==> related.tex <==
% SLU works
Existing work for leveraging web search and browsing behavior to spoken dialog systems mainly exploits offline information in the query-click logs. For instance, the web query-click graph has been used for domain detection~\cite{HakkaniEtAl2011_asru} and slot filling \cite{conf/interspeech/TurHHC11}. Recently, the idea of combining the power of internet browser and multi-modal input (e.g. speech, gesture, etc) is discussed in~\cite{Heck2012_slt} and implemented in~\cite{HeckEtAl2013_slam}. Our work is thus inspired by this idea and existing work on entity extraction from web search queries~\cite{Pasca:2007:WDN:1321440.1321536,Guo:2009:NER:1571941.1571989}.

%those work  usually starts with a set of seeds instances for each NE category, and then scan the query log to extract the corresponding contexts, which can then be used to identify new instances for each category.

%Human-computer addressee detection for conversational browsing \cite{conf/interspeech/ShribergSHH12} is also studied based on the web search logs. 

Our work is also in line with utilizing semantic graph for spoken language understanding. For example, \cite{HeckEtAl2013_interspeech} collect the entities from a knowledge base and and retrieve sentences containing those entities from Wikipedia to train the entity extraction classifiers. Similar approach is also utilized for relation extraction~\cite{HakkaniEtAl2013_icassp}, intent detection~\cite{HeckEtAl2012_slt} and slot filling\cite{TurEtAl2012_interspeech}.

% Entity extraction and relation extraction in web search query, however, the prediction is made on instance leval. Session information is not taken into consideration.



==> result.tex <==
\subsection{Query Session Likelihood}
Before evaluating our model on the two tasks, we first carry out experiments to validate the query session assumption. Concretely, we compute the loglikelihood of the query sessions in our training data based on Markov models with different orders, where higher order markov model considers longer history information.

Our experimental results show that Markov models with longer search history produce higher loglikelihood.

\subsection{Task 1: Web Query Semantic Parsing}
We first show that session history can improve semantic parsing accuracy for queries that match the most frequently occurring templates from \cite{Pound:2012:IKQ:2396761.2396803}. We test our model on the remaining 20\% of the IE log.


Due to the large size of the test data, it will be extremely time-consuming to acquire the gold standard annotation. Thus, we design a mechanism for automatic evaluation. We conduct ngram-based matching between the queries in the test set and the gazetteer obtained from Satori. We use the resulting labeling as the gold standard. 

Meanwhile, we assume our model only has the access to part of the gazetteer that appearing in the training data.

\todo{more details on relation and type matching}

\paragraph{Comparisons}

Maximum Entropy\cite{Curran:2003:LIN:1119176.1119200}

\paragraph{Discussion and Error Analysis}

\subsection{Task 2: Statistical Dialog Management}
By testing on the CB data and Netflix data, we also show that the model can be successfully used as a belief state update for a spoken dialog manager. As our model is trained on IE log and test on conversational data, this set of experiments demonstrate that our model has the ability to leverage the web search query-click log for dialog management, where additional human annotation for every new domain can thus be avoided.

\paragraph{Discussion and Error Analysis}

%\subsubsection{Conversational Browsing data}
%\subsubsection{Conversational Browsing on Netflix}




